P2P-NET: Bidirectional Point Displacement Net for Shape Transform

We introduce P2P-NET, a general-purpose deep neural network which learns geometric transformations between point-based shape representations from two domains, e.g., meso-skeletons and surfaces, partial and complete scans, etc. The architecture of the P2P-NET is that of a bi-directional point displacement network, which transforms a source point set to a target point set with the same cardinality, and vice versa, by applying point-wise displacement vectors learned from data. P2P-NET is trained on paired shapes from the source and target domains, but without relying on point-to-point correspondences between the source and target point sets. The training loss combines two uni-directional geometric losses, each enforcing a shape-wise similarity between the predicted and the target point sets, and a cross-regularization term to encourage consistency between displacement vectors going in opposite directions. We develop and present several different applications enabled by our general-purpose bidirectional P2P-NET to highlight the effectiveness, versatility, and potential of our network in solving a variety of point-based shape transformation problems.

==> limit.tex <==
%\revised{As we discussed above, the method can only learn mappings which are one-to-one or many-to-one in feature space, i.e., similar features cannot be mapped to dissimilar displacements.}

\rz{
We reiterate that our work is only a first attempt at designing a general-purpose shape transformation 
network. By no means should one expect P2P-NET to work effectively for all transformation tasks. The
network is inherently limited by its current architecture, training loss, and optimization scheme for the
network parameters. In what follows, we provide a non-exhaustive list of such limitations to explore the
behavior and limit of our method.

%The definition of a general-purpose shape transformation is wide. Currently, 
%the P2P-NET is not effective for all transformation tasks. 
%In the following discussion we explore the scope of the method and the limitations of P2P-NET. We start the discussion by stressing the non-trivial fact that the method was designed to learn the mappings in feature-spaces, rather than in point space. This means that for a given training set, the network learns to associate a  unique displacement vector with a point feature (in our case a PointNet feature). Thus, the network should be trained with examples where the implicit relation between point features and displacements is unambiguous. 

\vspace{-5pt}

%\paragraph{\bf{Ambiguous transformations}}
\paragraph{\bf{Ambiguous feature-to-displacement mapping.}}
%
In the absence of point-to-point correspondences between the training source and target shapes, P2P-NET
must learn point set transforms implicitly. Architecturally, P2P-NET first turns the input points into PointNET++
features. It then learns to map these point features to displacement vectors to minimize the training loss. As a 
result, P2P-NET should be trained with examples where the implicit relation between point features and 
displacements is {\em unambiguous\/}. The network should not be expected to learn to associate
points possessing similar features with {\em different\/} displacements.
%
In reality however, ambiguous feature-to-displacement mappings may be unavoidable for many transformation 
tasks. Moreover, they may be characteristic of an entire class of transformations or occur only for some shape 
pairs or only over a portion of the shapes. Any such case may potentially lead to failure cases by P2P-NET.

To provide a simple illustration, consider a 2D example of learning to map points
along a horizontal line to three vertical bars, as shown in Figure~\ref{fig:featureless}. We trained P2P-NET
using more than 1,000 examples of source and target pairs in random orientations and scales. However,
regardless of how many training examples we employed, the network still cannot map the mid-section
of the line to the middle bar since points near the mid-section all possess similar features. As shown in (a),
P2P-NET could only learn to associate these points with similar displacements. To verify that the crux of
the problem is the ambiguity, we added a small protrusion under the source line so that points near the
mid-section can be better distinguished by PointNET++ features. As can be seen in (b), now P2P-NET 
does a much better job of learning the proper transform.

% mappings can exist both in the point-level and in the shape-level. 
%
%At the point-level there is an inherent ambiguity when similar features should be associated with different displacements. To exemplified that clearly, we show a simple example in 2D, see Figure~\ref{fig:featureless}, where we learn to map from a section of straight line to three slanted sections. During training, a large number (over 1000 examples) of such source and target lines are employed in random orientations and scales. As shown in (a), the mapping from the source line to the middle line is extremely noisy. To understand this limitation let us analyze the details of this case. The features associated with the source line are quite similar around the its (featureless) center, while there is a richer variety of them close two endpoints. In the middle section, the network is required to associate  similar features to very different displacements toward the slanted line. This is quite hard. Note that we color the source line with by embedding the high-dimensional features to 1D using PCA. To better convince that the crux is in the featureless center section, we added a tiny geometry, a line segment below the middle of the line (see in (b)). Now the center of the line has a meaningful geometric features and PointNet generates different features about the source line. Then, as can be seen, the mapping is fixed, and P2P-NET succeed to learn noiseless displacement. 

\vspace{-5pt}

\paragraph{\bf{Ambiguous point transforms.}}
%
Some point set transforms may exhibit shape-level ambiguities, as shown in Figure~\ref{fig:boot}. The task is
to learn displacements from a shape silhouette to its interior details. The training set contains more
than 1,000 examples of adding details (via edge maps) to the {\em same\/} boot shape. To minimize the training loss, 
P2P-NET is only able to learn to displace to an {\em average\/} of the target points, leading to an erroneous outcome. 
%In this example,  trained on 1,000 pairs of salient object contours and edge maps extracted from the same boot images. 
 
%
%With an unknown camera view, the mapping from an object surface to its partial scan is also nondeterministic. The current P2P-NET is only able to deal with mapping from object surface to a scan with a known fixed camera view, as shown in Figure~\ref{fig:SSStransform}. To extend P2P-NET to a full-fledged scan completion network, a new factor of view must be introduced to map object surface to its incomplete scan deterministically.

\begin{figure}[t!]
	\centering
	\includegraphics[width=\linewidth]{figures/featureless}
	\caption{\rz{P2P-NET cannot be properly trained to map a horizontal line to three vertical bars since points near the mid-section possess similar point features. Our method fails to associate points with similar features with dissimilar displacements to clearly form the middle bar (a). However, a small added protrusion (b) can serve to disambiguate these point features, leading to different displacements to produce the middle bar. Colorings of the points reflect their features, after a 1D embedding using PCA.}}
%	In (b) a small segment is added below the source line causing the features in the middle section to vary. As can be seen, the predicted displacements are significantly enhanced.} 
	\label{fig:featureless}
\end{figure}
 
\begin{figure}[t!]
	\centering
	\includegraphics[width=0.9\linewidth]{figures/boot}
	\caption{P2P-NET cannot be properly trained for non-deterministic \rz{point set transforms}, e.g., adding details to a shape contour.}
	\label{fig:boot}
\end{figure}

\begin{figure}[t!]
	\centering
        \includegraphics[width=\linewidth]{figures/noisylines}
	\includegraphics[width=\linewidth]{figures/noisycross}
	\caption{\rz{P2P-NET cannot be trained to accurately and cleanly predict thin structures. Top: from a noisy input (red), as shown in (a), in contrast to the ground truth (b).
Bottom: from lower-resolution point set inputs.}}
	\label{fig:noisycross}
\end{figure}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.99\linewidth]{figures/profile_translation}
	\caption{\rz{P2P-NET cannot be trained to produce highly structured point sets cleanly, e.g., to transform between orthogonal profiles and parallel profiles for the same 3D shape (sofa on the right).}}
	\label{fig:profiletrans}
\end{figure}

%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=\linewidth]{figures/articulated}
%	\caption{{Predicted articulated transformations by P2P-NET (upper row) versus ground truth transformations (lower row) . From left to right, degrees of per part rotation angles are  30, 60, 90, 120.}}
%	\label{fig:articulated}
%\end{figure}

%\begin{figure}[t!]
%\centering
%
%\caption{P2P-NET cannot accurately predict a thin line(blue) from a noisy input (red), as shown in (a). See the comparison with ground truth in (b).}
%\label{fig:noisylines}
%\end{figure}

%\dc{figures 12 and 13 should be put in a single figures with a common caption}

\vspace{-5pt}

%\paragraph{\bf{Correlations among displacements}} 
\paragraph{\bf{Decorrelation of displacements.}} 
%
The training loss adopted by P2P-NET is predominantly a point-to-shape distance measure; it does not account for intrinsic
properties of the input shape. This immediately implies that P2P-NET would not learn such properties to possibly preserve 
them in the output point clouds. The point displacement vectors predicted by P2P-NET are not correlated or controlled by
the shape properties as the network predicts a displacement vector for each point independently.
%
%If the target points are correlated or have some coherent geometry, the network does not learn it. A simple example is demonstrated in 
Figure~\ref{fig:noisycross} shows that P2P-NET is unlikely to reproduce thin lines when all the training data contain clean,
thin line structures.
%
Figure~\ref{fig:profiletrans} shows that P2P-NET cannot be well trained to produce highly structured point sets, where the transform is
between orthogonal profiles and parallel profiles of the same shapes.
%
By the same token, P2P-NET is not part-aware, i.e., it is unlikely to preserve part structures of the input shapes. For examples, it
% Without correlations among displacements,  P2P-NET can predict the semantic of the target or say of the transformation. Similarly, P2P-NET 
cannot transform clean rooms into messy rooms, by displacing or adding point-set objects; only uncorrelated point-wise displacements 
are currently learned. 
}
